PrivacyRestore: Privacy-Preserving Inference in Large Language Models via Privacy Removal and Restoration

The widespread usage of online Large Language Models (LLMs) inference services has raised significant privacy concerns about the potential exposure of private information in user inputs to malicious eavesdroppers. Existing privacy protection methods for LLMs suffer from either insufficient privacy protection, performance degradation, or large inference time overhead. To address these limitations, we propose PrivacyRestore, a plug-and-play method to protect the privacy of user inputs during LLM inference. The server first trains restoration vectors for each privacy span and then release to clients. Privacy span is defined as a contiguous sequence of tokens within a text that contain private information. The client then aggregate restoration vectors of all privacy spans in the input into a single meta restoration vector which is later sent to the server side along with the input without privacy spans.The private information is restored via activation steering during inference. Furthermore, we prove that PrivacyRestore inherently prevents the linear growth of the privacy budget.We create three datasets, covering medical and legal domains, to evaluate the effectiveness of privacy preserving methods. The experimental results show that PrivacyRestore effectively protects private information and maintain acceptable levels of performance and inference overhead.

==> experiments.tex <==


\section{Experiments}

\subsection{Experiments setup}
\label{sec:exp_setting}

\textbf{Backbones.} We use Llama2-chat-7b \citep{touvron2023llama} as the LLM deployed on server side. 
We utilize BERT-base \cite{devlin2019bert} as the tiny model on the client side for attention-aware weighted aggregation mentioned in \S \ref{sec:res_agg}.
We also report results on larger LLMs such as Llama2-chat-13b \citep{touvron2023llama} and Llama3-8b-instruct \citep{llama3} in Appendix \ref{app:add_exp}.
% As for tiny model, we also consider BERT-large \cite{devlin2019bert} and the results are shown in \S \ref{}.

\textbf{Datasets.}
We mainly focus on protecting user inputs in medical diagnosis task. 
We consider symptoms in user inputs as privacy spans. 
In real-world scenarios, some symptoms may be highly sensitive, while others may be less sensitive or non-sensitive. 
Existing benchmarks such as PriDdxplus \citep{ars2022ddxplus} and NLICE \citep{al2023nlice} for the medical diagnosis task lack of privacy level of symptoms. 
We utilized GPT-3.5 \citep{ouyang2022training} to rate the privacy level for all possible symptoms in Ddxplus \citep{ars2022ddxplus} and NLICE\citep{al2023nlice} benchmark respectively.
The query prompt for rating privacy levels is shown in Appendix \ref{app:construction}.
Each symptom is rated from level 1 to level 5, with the definitions of privacy levels provided in Appendix \ref{app:level}. 
The sensitivity levels range from 1 (non-sensitive information) to 5 (highly sensitive information), with higher levels indicating increasing privacy levels.
Leveraging the source datasets (Ddxplus and NLICE) and incorporating privacy levels for symptoms, we curated two privacy-preserving datasets, named \textbf{Pri-Ddxplus} and \textbf{Pri-NLICE}, respectively. 
There are 149 and 70 types of privacy spans in Pri-Ddxplus and Pri-NLICE, respectively.
The detailed construction process and statistical information for two datasets are provided in Appendix \ref{app:dataset}.

\textbf{Metrics.}
The evaluation of privacy protection should consider both the performance, the effectiveness of privacy protection, and inference efficiency. 
% \revisejw{-> generation efficiency} 
% \revisezq{inference efficiency is a terminology.}
We evaluate the model's performance using two metrics: \textbf{MC1} and \textbf{MC2} \citep{lin2021truthfulqa}.
We assign each sample in Pri-Ddxplus and Pri-NLICE with four options, including one correct diagnosis and three incorrect ones. 
% To calculate MC1, we compute the accuracy of the option having the highest probability. 
To calculate MC1, we compute the accuracy, i.e., the proportion of questions answered correctly out of the total number of questions. 
We consider the option with the highest probability as the answer.
To calculate MC2, we compute the normalized probability of the true answer.
% Both metrics evaluate the diagnostic performance of the model.


To evaluate the effectiveness of privacy protection, we construct two commonly used privacy attacks targeted at LLMs, Prompt Injection Attack \citep{perez2022ignore, liu2023prompt} and Attribute Inference Attack \citep{mahloujifar2021membership, Li2022perna}. 
%\revisezd{\textbf{delete} We use the probability of a successful attack to reflect the effectiveness of privacy protection.
%The lower probability signifies the higher efficacy in preserving privacy.}
For prompt injection attack, attackers intercept the medical query and inject extra harmful prompts to induce the model to generate the privacy symptoms of patients.
If the model output contains privacy symptoms, we consider it as a successful attack. 
We compute the ratio of successful attacks, namely \textbf{ASR} (Attack Success Ratio).
For attribute inference attack, attackers intend to build up a simple multi-label classifier to map representations of the medical query into corresponding privacy symptoms. 
%Some incorrect symptoms may be predicted while some correct symptoms are ignored.
We compute the \textbf{F1} score of the classifier.
The lower the ASR and F1, the higher the effectiveness of privacy protection.


To evaluate inference efficiency, we measure latency and throughput. 
Latency is measured from the moment the user submits the query until the answer is generated.
As different samples have varying lengths, we calculate the average latency per sample and provide the average output length.
Latency is further divided into two parts: namely, \textbf{latency on server} side and \textbf{latency on client} side. 
The generation of meta restoration vector is conducted on the client side. 
Hence, it is necessary to investigate the latency of generating the meta restoration vector.
Lower latency indicates higher inference efficiency. 
In addition to latency, we compute the \textbf{throughput}, which denotes the number of tokens generated by the model per second.
Higher throughput indicates higher inference efficiency. 

Due to space limitations, implementation details are presented in Appendix \ref{app:imple_detail}.
%让chatgpt润色。
%The latency metric computes the average generation time using for one query.
%The throughput metric computes the average time cost for a single token during generation.


% For appendix
% \textbf{Implementation details.}
% For the fine-tuning process described in \S \ref{sec:res_corr}, we only train the restoration vectors and fix all other parameters of LLM. 
% The training is conducted for five epochs with a batch size of 8. 
% This process takes 4\textasciitilde5 hours on a single A100 GPU, which is a reasonable duration for retraining the model when new privacy spans are introduced. 
% % We set the learning rate as 1e-04 with 0.001 weight decay. 
% % We use the cosine learning rate scheduler with 0 warmup ratio.

% For the classifier used in the attribute inference attack, we employ a 2-layer Multilayer Perceptron (MLP) as the classifier, following the approach in \cite{Li2022perna}.
% The classifier is trained on the same dataset used for restoration vector training. 
% The classifier takes the query representation as the input and predicts whether the query contain specific symptoms. 
% We regard the meta restoration vector as the query representation. 
% The other methods in \S \ref{sec:baseline} do not have obvious representations associated with the privacy spans. 
% We utilize the hidden state of the last token from the last layer of LLM as the query representation. 
% % We training the classifiers for ten epochs using a batch size of 32. 
% % We set the learning rate as 3e-5 with no weight decay. 
% % We use the linear learning rate scheduler with 100 warmup steps.
% % \revisezq{mention training data of attribute inference.}

% Differential privacy \citep{qu2021natural} use $\eta$ to control the strength of injected noise.
% Smaller $\eta$ provides stronger privacy protection but results in significant performance degradation.
% %As shown in \cite{li2023privacy}, the range of $\eta$ is from 75 to 175 for acceptable performance degradation .
% %For DP based baseline in Section \ref{sec:baseline}, we set the $\eta$ to 75 considering better privacy protection. 
% As shown in \cite{li2023privacy}, $\eta$ ranges from 75 to 175. A lower value represents a higher level of privacy protection. 
% For the DP based methods, we set $\eta$ to 75 to prioritize privacy protection.
% % \revisezq{why 75, following any paper? what is the range of $\eta$?}
% For noise injection regarding the single restoration vector case mentioned in \S \ref{sec:res_agg}, we use the same $\eta=75$ to maintain a consistent noise level.

% To evaluate inference efficiency, we use the greedy search decoding strategy and restrict the max generation length to 64.
% For top-K heads selector, we following the setting of \cite{li2023iti} and set K to 48.
% All of our experiment is conducted on the NVIDIA A800.

% For appendix


















% \revisezq{mention the noise rate of dp.}
% \revisezq{need to mention the training time of restoration vectors.}
% \cite{Lin2019end}
% Existing benchmarks \citep{zhong2018dx, Lin2019end, yu2018samy, ars2022ddxplus, al2023nlice}
% Previous research on Automatic Medical Diagnosis has primarily focused on enhancing the performance of diagnostic models, such as \cite{wei2018task, hong2021bayesian, Hong2021efficient}. 
% Existing benchmarks \citep{zhong2018dx, Lin2019end, yu2018samy, ars2022ddxplus} solely comprise patients' symptoms and corresponding diagnosis data, without incorporating the privacy levels associated with different symptoms.
% For instance, the symptom \textit{coughing up blood} is typically more private than \textit{pain}.
% We construct a novel dataset named \textbf{Privacy DDXPlus (PriDDXPlus)} specifically tailored for addressing privacy-preserving challenges in medical diagnosis.

% We utilized GPT-3.5 \citep{ouyang2022training} to assess the privacy levels of all possible symptoms in DDXPlus \citep{ars2022ddxplus}, ranging from non-sensitive to highly sensitive. 
% Detailed definitions of the privacy levels are provided in Table \ref{tbl:privacy_level}.
% Higher level indicates greater sensitivity, and there are five levels in total.
% The assessing prompt template is shown in Figure \ref{fig:privacy_level}.

% The initial DDXPlus dataset is extensive, and we observed that for most samples, providing only non-sensitive symptoms often yields diagnosis outputs similar to those obtained when all symptoms are provided.
% However, in real world, sensitive symptoms often play an vital role in diagnosis. 
% Our dataset should include samples where privacy symptoms are crucial for diagnosis outcomes.
% We filter out data with high KL divergence in the model output distribution between queries containing all symptoms and those containing only non-sensitive symptoms.
% Higher KL divergence indicates that the absence of sensitive symptoms may lead to different or even incorrect diagnosis outcomes.
% The detail statistics of PriDDXPlus are present in Section \ref{sec:dataset}.
% Some Examples of PriDDXPlus are given in \ref{sec:example}.

% \subsection{Evaluation Metrics}
% % We evaluate the effectiveness of the proposed CPP-Resin on PriDDXPlus considering both diagnostic utility and privacy protection.

% \textbf{Diagnostic Utility} assesses whether the model can correctly distinguish the actual pathology of a patient and output the correct diagnosis.
% As shown in Figure \ref{fig:example}, each query is assigned four options, including one correct diagnosis and three incorrect ones.
% Inspired by \cite{lin2021truthfulqa}, we evaluate the diagnostic utility by computing the likelihood of the correct diagnosis conditional on the query.
% There are two variants of evaluation indicators, namely \textbf{MC1} and \textbf{MC2}. 
% In MC1, only the correctness of the option with the highest probability is considered, whereas in MC2, the normalized probability of the true answer is calculated.
% Detail explanations of both two indicator are shown in \ref{}.

% \textbf{Privacy Protection} evaluates the model's ability to prevent privacy leakage under various attacks.
% We consider two commonly used attacks, Prompt Injection Attack \citep{perez2022ignore, liu2023prompt} and Attribute Inference Attack \citep{pan2020privacy, mahloujifar2021membership}. 
% Prompt injection attack (PIA) intercepts patients' query and injects extra harmful prompts to induce model output the privacy symptoms of patients. 
% An attack is considered successful when the model's output contains one of the patients' privacy symptoms. 
% For PIA, we calculate the attack success ratio, denoted as \textbf{ASR}.
% Attribute inference attack (AIA) intend to build up simple neural networks mapping vector representations of patients' query into various privacy symptoms. 
% These neural networks are called attribute classifiers, and all previous work performs classification using contextualized embeddings from LLM.
% Especially, in our CPP-Resin, attribute inference attack is possibly used to attack the complex intervention vector calculated by Equation \ref{eq:newComplex}.
% For AIA, we calculate the F1 score of the attribute classifiers, denoted as \textbf{Attack F1 (AF)}.
% Both ASR and AF serve as indicators of the model's robustness against privacy attacks.




% \subsection{Implementation Details}
% \textbf{Models}. We employ Llama2-chat-7b and its 13b variant \citep{touvron2023llama} as the base model suffering the privacy attacks. We also report the results on Llama3-8b-instruct. 
% For small client models mentioned in \ref{sec:inter_over}, we use bert-base and bert-large \cite{}. 
% For simple classifier of AIA attack mentioned in \ref{}, we use two .

% \textbf{Training Details}.

\subsection{Compared Methods}
\label{sec:baseline}
To demonstrate the effectiveness of our method, we compare our model with the following baselines:
\textbf{No Protection}. 
The client does not provide any protection for patient's queries and sends the intact queries to the servers. 
Since the query is intact, the model's performance is not affected.
It provides a theoretical upper bound of the model's performance. 
However, it suffers from the privacy leakage.
\textbf{Direct Removal}.
%Actually, when users utilize the LLM service, they clearly know which span of the query is the privacy span. 
The user directly deletes all privacy spans in the input and submits it to the LLM. 
\textbf{DP}. 
Differential privacy method \citep{qu2021natural} apply text-to-text privatization \citep{feyisetan2020privacy} on user inputs, which injects noise into tokens' embedding and find the nearest tokens to replace the initial tokens. 
The text-to-text privatization is applied on all tokens in the input. 
The LLM backbone of DP method is frozen. 
%Without knowing the specific privacy spans, DP replaces all tokens in queries to prevent attackers from stealing private information. 
%As revealed by research \cite{li2023Privacyin}, DP provides privacy guarantees for private data privacy but suffers from performance degradation. 
\textbf{DP on Privacy Spans}.
The client employs the text-to-text privatization \citep{feyisetan2020privacy} on privacy spans, rather than the entire query.
% \revisezq{Why do not consider SMPC as the baselines.} 
SMPC 
% \revisezq{If SMPC is not a baseline, then do not need bold font. } 
methods suffer from huge inference time overhead. We do not include them as a baseline. 
% compared merhods 要提一句，为什么不和smpc方法比，因为他们的效果和隐私保护程度是最高的，只关注inference efficiency。

The settings in the ablation study of PrivacyRestore are shown as follows.
\textbf{w/o Top-K Heads Selector.} 
We remove the Top-K heads selector in PrivacyRestore. 
We randomly select K heads from $\mathcal{H}_a$ to form the head set $\mathcal{H}_c$.
\textbf{w/o Restoration Vectors Training.} 
We eliminate the training process and do not use trainable restoration vectors. 
We use an activation steering method called ITI \cite{li2023iti} to obtain the restoration vectors of each privacy span. 
%For each privacy span $s$, we compute the outputs of each attention head for queries after the removal of $s$ and for queries without removal. 
%We then calculate the mean of the head outputs for queries with removal and the mean of the head outputs for queries without removal. 
%The restoration vector for $s$ is computed by taking the difference between these two mean outputs.
%\revisezq{Can we say we use ITI to get the restoration vectors, save some space?}
\textbf{w/o AWA.} 
We remove the attention-aware weighted aggregation component. The meta restoration vector is computed as an equally weighted sum of restoration vectors of all privacy spans.  
%\revisezq{Ignoring the importance weights of different privacy spans, we obtain the meta restoration by equally adding the restoration vectors of all privacy spans. }




\begin{table*}
	\centering
        \def\arraystretch{1.5}
	\resizebox{1\textwidth}{!}{
		\begin{tabular}{l   c cccc  cccc  cccc  cccc}
			\toprule
            % \cmidrule(lr){1-18}
            \multicolumn{17}{c}{\textbf{Pri-Ddxplus}} \\
            % \cmidrule(lr){1-18} 
            \midrule
		  \multirow{2}{*}{Methods} & \multirow{2}{*}{Privacy} &  \multicolumn{4}{c}{$\geq \text{Level 2}$} &  \multicolumn{4}{c}{$\geq \text{Level 3}$} &  \multicolumn{4}{c}{$\geq \text{Level 4}$} &  \multicolumn{4}{c}{$\geq \text{Level 5}$}\\ 
            \cmidrule(lr){3-18}
			& & MC1 $\uparrow$  & MC2 $\uparrow$ & ASR $\downarrow$ &  \multicolumn{1}{c|}{F1 $\downarrow$}    &   MC1    & MC2  & ASR & \multicolumn{1}{c|}{F1}   &   MC1    & MC2  & ASR & \multicolumn{1}{c|}{F1} &   MC1 & MC2  & ASR & F1\\ 
            \midrule
            No Protection & $\times$ & 86.83 & 85.13 & 100.00 & \multicolumn{1}{c|}{12.30}
            & 86.83 & 85.13 & 100.00 & \multicolumn{1}{c|}{12.30}
            & 86.83 & 85.13 & 100.00 & \multicolumn{1}{c|}{12.30}
            & 86.83 & 85.13 & 100.00 & 12.30 \\

            
            Direct Removal  &\checkmark & 33.31 & 33.49 & 45.19 & \multicolumn{1}{c|}{7.27} 
            & 63.20 &59.47 & 24.79 &\multicolumn{1}{c|}{4.54} 
            &78.24 & 75.66 &10.20 &\multicolumn{1}{c|}{1.23} 
            &86.24 &84.45 &0.58 &1.58 \\


            DP \citep{qu2021natural} &\checkmark & 41.83 & 40.61 & 70.69 & \multicolumn{1}{c|}{6.28}
            & 41.83 & 40.61 & 70.69 & \multicolumn{1}{c|}{6.28}
            & 41.83 & 40.61 & 70.69 & \multicolumn{1}{c|}{6.28}
            & 41.83 & 40.61 & 70.69 & 6.28  \\
            
            
            DP on Privacy Spans &\checkmark & 41.83 &40.61 & 70.69 &\multicolumn{1}{c|}{6.28} 
            &65.59 &63.01 &43.44 &\multicolumn{1}{c|}{3.62} 
            &78.37 &75.68 &8.58 &\multicolumn{1}{c|}{1.33} 
            &86.44 &84.55 &0.51 &1.71 \\

            
            \rowcolor{lightgray!45} 
            \textbf{PrivacyRestore}  &\checkmark & \textbf{61.78} & \textbf{61.13} & 41.18 & \multicolumn{1}{c|}{5.81}
            & \textbf{75.40} & \textbf{72.83} & 22.27 & \multicolumn{1}{c|}{0.25}
            & \textbf{84.89}& \textbf{84.09}& 8.56& \multicolumn{1}{c|}{\textbf{0.00}}
            & \textbf{87.73}& \textbf{85.96}& 0.51& \textbf{0.00}  \\

            
            \rowcolor{lightgray!45}
            w/o Top-K Heads Selector &\checkmark & 21.04 & 22.19 & 49.96 & \multicolumn{1}{c|}{5.94}
            & 27.82& 27.87& 11.87& \multicolumn{1}{c|}{26.51}
            & 67.59 & 67.45 & \textbf{3.55} & \multicolumn{1}{c|}{42.35}
            & 85.86& 83.96& \textbf{0.00} & 35.8  \\

            
            \rowcolor{lightgray!45}
            w/o Restoration Vectors Training &\checkmark & 41.05& 39.15 & 37.44 & \multicolumn{1}{c|}{5.82}
            & 48.58 & 45.23 & 27.63 & \multicolumn{1}{c|}{0.58}
            & 64.36 & 64.11 & 12.39 & \multicolumn{1}{c|}{\textbf{0.00}}
            & 85.92 & 84.14 & 0.12 & \textbf{0.00}  \\

            
            \rowcolor{lightgray!45}
           w/o AWA &\checkmark &44.35 & 43.26 & \textbf{3.74} & \multicolumn{1}{c|}{\textbf{0.00}}
           & 68.62& 65.95 & \textbf{3.87} & \multicolumn{1}{c|}{\textbf{0.00}}
            & \textbf{84.89}& 84.07& 13.36 & \multicolumn{1}{c|}{\textbf{0.00}}
            & \textbf{87.73}& 85.95 & 0.06& \textbf{0.00}  \\

            
            \midrule 

            \multicolumn{17}{c}{\textbf{Pri-NLICE}} \\
            % \cmidrule(lr){1-18} 
            \midrule
		  \multirow{2}{*}{Methods} & \multirow{2}{*}{Privacy} &  \multicolumn{4}{c}{$\geq \text{Level 2}$} &  \multicolumn{4}{c}{$\geq \text{Level 3}$} &  \multicolumn{4}{c}{$\geq \text{Level 4}$} &  \multicolumn{4}{c}{$\geq \text{Level 5}$}\\ 
            \cmidrule(lr){3-18}
			&& MC1 $\uparrow$ & MC2 $\uparrow$ & ASR $\downarrow$ &  \multicolumn{1}{c|}{F1 $\downarrow$}   &   MC1    & MC2  & ASR & \multicolumn{1}{c|}{F1}   &   MC1    & MC2  & ASR & \multicolumn{1}{c|}{F1} &   MC1 & MC2  & ASR & F1\\ 
            \midrule
             No Protection & $\times$ & 76.64 & 75.80 & 77.78 & \multicolumn{1}{c|}{75.87}
            & 76.64 & 75.80 & 77.78 & \multicolumn{1}{c|}{75.87}
            & 76.64 & 75.80 & 77.78 & \multicolumn{1}{c|}{75.87}
            & 76.64 & 75.80 & 77.78 & 75.87 \\

            
            Direct Removal & \checkmark & 58.58 & 55.18 & 2.27 & \multicolumn{1}{c|}{23.86}
            & 64.52 & 61.63 & 0.00 & \multicolumn{1}{c|}{20.49}
            & 73.73 & 72.12 & \textbf{0.00} & \multicolumn{1}{c|}{3.84}
            & 74.36 & 72.85 & \textbf{0.00} & 1.1 \\


            DP \citep{qu2021natural} & \checkmark & 59.21 & 56.12 & \textbf{0.00} & \multicolumn{1}{c|}{18.72}
            & 59.21 & 56.12 & \textbf{0.00} & \multicolumn{1}{c|}{18.72}
            & 59.21 & 56.12 & \textbf{0.00} & \multicolumn{1}{c|}{18.72}
            & 59.21 & 56.12 & \textbf{0.00} & 18.72\\

            
            DP on Privacy Spans & \checkmark & 37.87 & 38.98 & 0.50 & \multicolumn{1}{c|}{20.86}
            & 48.10 & 47.17 & 0.01 & \multicolumn{1}{c|}{18.66}
            & 72.22 & 70.40 & \textbf{0.00} & \multicolumn{1}{c|}{3.30}
            & 73.48 & 71.70 & \textbf{0.00} & 0.79 \\

            
            \rowcolor{lightgray!45} 
            \textbf{PrivacyRestore} & \checkmark & \textbf{79.54} & \textbf{78.81} & 0.25 & \multicolumn{1}{c|}{\textbf{0.00}}
            & \textbf{78.66} & \textbf{77.44} & 0.12 & \multicolumn{1}{c|}{\textbf{0.12}}
            & \textbf{76.64} & \textbf{75.35} & 0.37 & \multicolumn{1}{c|}{6.52}
            & \textbf{75.88} & \textbf{74.98} & \textbf{0.00} & \textbf{0.00} \\

            
            \rowcolor{lightgray!45}
            w/o Top-K Heads Selector & \checkmark & 71.46 & 67.92 & 5.05 & \multicolumn{1}{c|}{12.79}
            & 70.20 & 69.30 & 0.75 & \multicolumn{1}{c|}{18.61}
            & 72.22 & 70.44 & 0.13 & \multicolumn{1}{c|}{\textbf{2.17}}
            & 71.46 & 70.53 & \textbf{0.00} & 1.29 \\

            
            \rowcolor{lightgray!45}
            w/o Restoration Vectors Training & \checkmark & 54.16 & 50.93 & 5.42 & \multicolumn{1}{c|}{27.83}
            & 61.99 & 58.77 & 0.25 & \multicolumn{1}{c|}{22.63}
            & 72.97 & 71.73 & 0.50 & \multicolumn{1}{c|}{7.36}
            & 72.97 & 72.61 & \textbf{0.00} & 6.38 \\

            
            \rowcolor{lightgray!45}
           w/o AWA & \checkmark & 76.76 & 74.61 & 0.12 & \multicolumn{1}{c|}{28.36}
            & 78.4 & 77.31 & 0.12 & \multicolumn{1}{c|}{22.55}
            & 76.63 & 75.33 & 0.37 & \multicolumn{1}{c|}{7.36}
            & \textbf{75.88} & \textbf{74.98} & \textbf{0.00} & 6.38 \\
            
            \midrule 

  
		\end{tabular}
  
	}

 \caption{
%Comparison of the model's performance and the effectiveness of privacy protection among compared methods on Pri-Ddxplus and Pri-NLICE dataset. 
%MC1 and MC2 indicate the model's performance, with higher values representing better performance.
%ASR and F1 indicate the effectiveness of privacy protection, with lower values representing better performance.
%$\geq \text{Level k}$ means that we apply protection for symptoms with a privacy level greater than or equal to k. 
%The privacy column shows whether the method applies protection to the user's query.
Comparison of the model performance and the effectiveness of privacy protection among the compared methods on the Pri-Ddxplus and Pri-NLICE datasets on Llama2-chat-7b. MC1 and MC2 metrics indicate the model's performance, with higher values representing better performance. 
ASR and F1 metrics measure the effectiveness of privacy protection, with lower values indicating better performance. 
The ``$\geq \text{Level} \; j$'' column indicates that privacy protection is applied to symptoms with a privacy level greater than or equal to $j$. The ``Privacy'' column shows whether the method applies privacy protection to the user input or not.
The best model performance and privacy protection are marked in bold, excluding the No Protection method, as it does not provide any privacy protection.
}
\label{table_avg_acc}
\end{table*}



\subsection{Main Results}
As shown in Table \ref{table_avg_acc}, we evaluate the performance and effectiveness of privacy protection on two datasets. 
Since the No Protection method does not use any protection and the DP method injects noise into all tokens in the query, the outcomes of both methods are independent of the privacy level.
As shown in the first row of the upper and lower parts, the No Protection method achieves the upper bound of the MC1 and MC2 but suffers from privacy leaking problems on two datasets. 
% Hence, there is a need to explore how to protect privacy.

% 讲一下 level1-5的区别
Direct Removal method serves as a strong competitor in privacy protection but suffers from model performance degradation.
% , as indicated by the second rows of both two table parts.
% Non-zero ASR and F1 imply that attackers may sometimes deduce the removed privacy symptoms from the other context but it is very hard.
The lower level means more privacy symptoms were removed and the performance degradation is more obvious.  
% DP on the entire query or on privacy spans replaces the removal operation with injecting noise.
% They can partially recover the model performance but their performance is still significantly lower than the No Protection method.
% Their privacy protection capability is weaker than Direct Removal method.  
The performance of DP and DP on Privacy Spans is significantly lower than the No Protection method, and their privacy protection capability is weaker than Direct Removal methods.

Compared to DP based methods, PrivacyRestore achieves significant improvements in model performance with even lower ASR and F1. 
The model performance is comparable to the No Protection method.
Moreover, sometimes PrivacyRestore even outperforms the No Protection method, as demonstrated in the $\geq \text{Level 5}$ case on Pri-Ddxplus dataset and the $\geq \text{Level 2}$, $\geq \text{Level 3}$, $\geq \text{Level 5}$ cases on Pri-NLICE dataset.
This suggests that using the restoration vectors for the corresponding privacy symptoms can sometimes be more beneficial for model inference than including the symptom directly in the query context.
Surprisingly, Privacy Protection achieves better privacy protection ability than Direct Removal with lower ASR and F1 on both datasets.
It indicates that applying restoration vectors in model inference can effectively prevent attackers from stealing the privacy symptoms.

We also provide the results after removing the Top-K Heads Selector, Restoration Vectors Training and Attention-aware Weighted Aggregation (AWA) components respectively.
After removing Top-K Heads Selector and Restoration Vectors Training, both the model performance and effectiveness of privacy protection are weakened. 
% After removing the AWA component, we observe a slight improvement in privacy protection with a significant degradation of model performance.
% This improvement in privacy protection may be attributed to our assignment of high importance weights to certain symptoms in the meta restoration vectors, making these symptoms easier to be detected when they occur.
After removing the AWA component, both the model performance and privacy protection capability decrease (except for slight changes in ASR), which indicates the effectiveness of AWA component.








\subsection{Inference Efficiency}
We compare the inference efficiency of the initial model and PrivacyRestore on Llama2-chat-7b in Table \ref{tbl:table_gen}. 
On the server side, PrivacyRestore needs to edit the attention heads using the meta restore vector during model inference on the server as shown in Eq \ref{eq:MHA-inter-1}.
These operations are fast and only bring 8\%-13\% overhead on the server, as shown in the ``Latency on Server'' column.
On the client side, PrivacyRestore needs to generate the meta restoration vector for uses. 
%The collaborative model for the aggregation operation is smaller compared to the model deployed on the server. 
%Therefore, 
The latency on the client side is relatively minor compared to the latency on the server, as depicted in the ``Latency on Client'' column.
As shown in the `Throughput'' column, PrivacyRestore can achieve nearly 80\% of the throughput of the original model. 

\begin{table*}[htbp]
	\centering
        \def\arraystretch{1.2}
	\resizebox{0.90\textwidth}{!}{
		\begin{tabular}{l   c  c c c c  c c }
			\toprule
   

            \multicolumn{8}{c}{\textbf{Pri-Ddxplus}} \\
            \midrule 
            \multirow{2}{*}{Methods}  & \multirow{2}{*}{Avg. Output Length} & \multirow{2}{*}{Latency on Server} & \multicolumn{4}{c}{Latency on Client} & \multirow{2}{*}{Throughput} \\
             \cmidrule(lr){4-7}
             & & & \multicolumn{1}{c|}{$\geq \text{Level 2}$}  
             & \multicolumn{1}{c|}{$\geq \text{Level 3}$} 
             & \multicolumn{1}{c|}{$\geq \text{Level 4}$}
             & $\geq \text{Level 5}$ &  \\
            \midrule
             Initial & 8.44 & 531.05 & - & - & - & - & 15.9 \\
             \multirow{1}{*}{\textbf{PrivacyRestore}} & \multirow{1}{*}{9.14} &  601.46 &  109.84 &  88.52 &  89.07 &  145.63 & \multirow{1}{*}{12.83 (\textbf{81\%})} \\
             % &  & \cellcolor{lightgray!45} & \cellcolor{lightgray!45} (15.44\%)
             % & \cellcolor{lightgray!45} (12.82\%) & \cellcolor{lightgray!45} (12.89\%) &
             % \cellcolor{lightgray!45} (19.49\%) &  & 
             \midrule

             \multicolumn{8}{c}{\textbf{Pri-NLICE}} \\
                \midrule 
            \multirow{2}{*}{Methods}  & \multirow{2}{*}{Avg. Output Length} & \multirow{2}{*}{Latency on Server} & \multicolumn{4}{c}{Latency on Client} & \multirow{2}{*}{Throughput} \\
             \cmidrule(lr){4-7}
             & & & \multicolumn{1}{c|}{$\geq \text{Level 2}$}  
             & \multicolumn{1}{c|}{$\geq \text{Level 3}$} 
             & \multicolumn{1}{c|}{$\geq \text{Level 4}$}
             & $\geq \text{Level 5}$ &  \\
            \midrule
             Initial & 6.56  & 462.04 & - & - & - & - & 14.2 \\
             \multirow{1}{*}{\textbf{PrivacyRestore}} & \multirow{1}{*}{6.56} &  506.27 &  91.03 &  86.84 &  79.34 &  79.25 & \multirow{1}{*}{11.12 (\textbf{78\%}}) \\
             % &  &  &  (15.24\%)
             % & \cellcolor{lightgray!45} (14.64\%) & \cellcolor{lightgray!45} (13.54\%) &
             % \cellcolor{lightgray!45} (13.53\%) &  & 

             \midrule
  
		\end{tabular}
	}
 \caption{Comparison of inference efficiency between original model (Llama2-chat-7b) and PrivacyRestore. Latency was measured in milliseconds (ms), and throughput denotes tokens per second. The \textbf{bold} number represents the ratio of PrivacyRestore's throughput to that of the original model. }
 \label{tbl:table_gen}
\end{table*}

% \subsection{}


==> fig/multi_plots/diff_ratio.tex <==



% \begin{figure*}[!t]
% \centering 
%     \subfigure[Embedding Inverse Attack] {
%      \label{fig:grow_pi}     
%     \includegraphics[width=0.25\columnwidth]{fig/plots/embedding_inverse_rouge.pdf}  
%     }    
%     % \hfill
%      \subfigure[Attribute Inference Attack] {
%      \label{fig:grow_ai}     
%     \includegraphics[width=0.25\columnwidth]{fig/plots/attribute_inference_PR2.pdf}  
%     }    
%     \vspace{-6pt}
%     \caption{Results of Embedding Inverse Attack and Attribute Inference Attack under different privacy span ratio $\alpha$ across three privacy-preserving datasets.}
%     \label{fig:different_ratios}
% \end{figure*}


\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-1.5\baselineskip}
  \begin{center}
    \subfigure[\centering Embedding Inverse Attack] {
     \label{fig:grow_pi}     
    \includegraphics[width=0.22\columnwidth]{fig/plots/embedding_inverse_rouge.pdf}  
    }    
    % \hfill
     \subfigure[Attribute Inference Attack] {
     \label{fig:grow_ai}     
    \includegraphics[width=0.22\columnwidth]{fig/plots/attribute_inference_PR2.pdf}  
    }    
  \end{center}
  \vspace{-1.2\baselineskip}
  \caption{Results of PrivacyRestore under embedding inverse attack and attribute inference attack under different privacy span ratios $\alpha$ on three datasets.}
  \label{fig:different_ratios}
  \vspace{-0.75\baselineskip}
\end{wrapfigure}


==> method2.tex <==

\section{Threat Model}
\label{sec:threat_model}
We consider a threat model involving two parties: a server that holds the LLM weights and a client with user inputs containing privacy spans. 
These privacy spans could be patient symptoms in the medical domain or case details in the legal field, which may leak private information.
The server provides services via an API, where the client transmits inputs and receives responses, while the LLM weights remain private. 
Our task is to protect these private spans in user inputs from being intercepted to the adversaries.


\section{The Proposed Method}
The fundamental idea of PrivacyRestore is removing privacy spans in user inputs and restoring privacy information via activation steering \citep{li2023iti,turner2023activation, hernandez2023inspecting} during model inference.

%This section presents the details of our framework \textbf{PrivacyRestore} based on Compensatory Privacy Protection. 
%PrivacyRestore not only prevents privacy breaches but also maintains the robust capabilities of a large language model. 
We first introduce the threat model in \S \ref{sec:threat_model} and the overview of PrivacyRestore in \S \ref{sec:overview} respectively. 
Subsequently, we provide detailed illustrations of the three components of PrivacyRestore, namely, edited attention heads identification, restoration vectors training, and restoration vectors aggregation. 
We will introduce the inference process in \S \ref{sec:infer}. 
Additionally, we introduce possible attack scenarios that PrivacyRestore might encounter in Appendix \ref{app:defense}. 
% \begin{figure*}[htbp]

% \centering
% \includegraphics[width=1\textwidth]{fig/definition.pdf}
% \caption{
% Different methodologies can be used to address privacy concerns when utilizing Language Model (LLM) as a diagnostic provider. (a). \textbf{No Protection} provides no safeguard for patients' descriptions of privacy spans or medical history. (b). \textbf{Directly Mask} masks privacy information about patients within descriptions; (c). \textbf{Different Privacy} inject noise into descriptions to avoid privacy leaking. (d). \textbf{PrivacyRestore} also masks privacy information but transfers restoration compass to restore performance during LLM inference phase. 
% }

% \label{fig:definition}
% \end{figure*}





% \subsection{Attack Scenario and Existing Methodologies}
% LLM service providers commonly receive users' queries and provide LLM responses in return. 
% This paradigm has sparked widespread concerns regarding users' privacy, particularly in the medical response field. 
% According to \cite{fansi2022ddxplus}, possible privacy information for medical response may be privacy spans and antecedents (describing the patient’s medical history and potential risk factors). 
% Patients need to tranfer descriptions about their privacy spans and antecedents to LLM servers, then attackers (eavesdroppers) can easily obtain some sensitive information containing in these description, as depicted in Figure \ref{fig:definition}. 

% As shown in Figure\ref{fig:definition}, several methodologies can be utilized to protect patients' privacy information. Directly Masking privacy information in patients' descriptions can simply but effectively avoid privacy leaking. 
% However, lacking of these privacy information will degrade LLMs' performance. Incomplete descriptions will produce wrong response result or even no response. 
% Some recent work has applied DP (differential privacy) in privacy protection for encoder-only language model, such as Bert \citep{devlin2018bert} and T5 \citep{raffel2020exploring}. 
% DP injects noise into patients' descriptions, preventing attackers from discerning the original text.
% Nonetheless, small noise only provides weak privacy protection where attacker can recover perturbed tokens. And large noise can cause severe damage to model performance. There exists a trade-off problem between privacy protection and model utility.

% 联邦学习+同态加密
% Federated learning allows models to be trained across distributed devices without exchanging raw data, thus preserving privacy while maintaining performance. Differential privacy adds noise to the data to prevent individual data points from being exposed, ensuring privacy without significantly compromising model performance. Meanwhile, homomorphic encryption enables computations to be performed directly on encrypted data, preserving privacy throughout the computation process.

%讲述一下病症mask

\subsection{The Overview of PrivacyRestore}
\label{sec:overview}
% 画图
The fundamental idea of PrivacyRestore is removing privacy spans in user inputs and restoring privacy information via activation steering \citep{li2023iti,turner2023activation, hernandez2023inspecting} during model inference. An overview of PrivacyRestore is depicted in Figure \ref{fig:algorithm}. 
%PrivacyRestore can protect private information while maintaining acceptable levels of performance and inference efficiency.
%The fundamental idea of PrivacyRestore lies in the notion that directly masking privacy information can \revisezd{effectively prevent privacy leakage.}
% serve as an effective defense against attacks. 
%Moreover, by devising mechanisms to compensate for lacking private information during inference, mitigating diagnostic performance degradation becomes feasible. 

% \revisezd{
% \revisezq{Move to the caption.}
% PrivacyRestore consists of three parts:
% (1) \textbf{Edited Attention Heads Identification.} 
% We will use probes \cite{alain2016understanding, tenney2019bert, belinkov2022probing} to identify attention heads that can distinguish whether the input text contains private spans and select a common set of attention heads for different private spans based on the accuracy of the probes.
% %and obtain representations of privacy spans from the activation space on attention heads. 
% (2) \textbf{Restoration Vectors Training.}
% We train restoration vectors with the aim of better restoring privacy information. 
% %and \revisezq{making predictions closer to those given complete privacy spans.}
% %没有privacy
% After that, we construct a Restoration Bank which consists of restoration vectors and common top-K attention head set. 
% %\revisezd{Representations of privacy tokens in (1) will be collected into a restore bank to initialize restoration vectors, which implicitly contain privacy information.}
% (3) \textbf{Restoration Vectors Aggregation.}
% We propose an \revisezq{attention-aware method to collaboratively aggregate different restoration vectors.}
% \revisejw{
% PrivacyRestore consists of three parts:
% (1) \textbf{Edited Attention Heads Identification.} 
% (2) \textbf{Restoration Vectors Training.}
% (3) \textbf{Restoration Vectors Aggregation.}
% % avoiding interference with each other.
% The first two processes are conducted on the server side while the last process is conducted on the client side. 
% In the subsequent sections, we elucidate the details of three components.
% }



%\revisezd{In the above steps, only the LLM inference process and the training process in Restoration Vectors Training are performed in the server, while the rest are performed in the client.}
% According to \cite{elhage2021mathematical} and \cite{vaswani2017attention}, the transformer architecture consists of repeated transformer layers, each comprising multi-head attention (MHA) and multilayer perceptron (MLP) modules. 
% Moreover, MHA modules are responsible to capture relationship between the current token and its surrounding context.
% Therefore, directly masking privacy information within context may lead to improper or insufficient relationships due to incomplete context fed into MHA modules.  
% MHA modules can be expressed as:
% \begin{eqnarray}
%     \label{eq:MHA}
%     x_{l+1}^{h} &=& Attn_{l}^{h}(x_{l}^{h}), \\
%     x_{l+1} &=& MHA(x_{l}), \\
%     MHA(x_{l}) &=& [x_{l+1}^{1}; x_{l+1}^{2};...;x_{l+1}^{H}] \cdot W^{O},  
% \end{eqnarray}
% where $x_{l}$ is the hidden state in the $l$th layer, $x_{l+1}^{h}$ is the hidden state on the $h$th head in the $l$th layer, $MHA$ is the multi-head attention function and $Attn_{l}^{h}$ is the attention operation for the $h$th head in the $l$th layer.

% Inspired by \cite{li2024inference}, we inject restoration into hidden state in MHA modules to restore lacking private information:
% \begin{eqnarray}
%      % \label{eq:MHA-inter-2}
%      % \mathcal{I}_{l}^{h} &=& \sum_{s\in\mathcal{S}}i_{s}^{l,h}, \\
%      \label{eq:MHA-inter-1}
%      x_{l+1}^{h} &=& Attn_{l}^{h}(x_{l}^{h}) + \mathcal{I}_{l}^{h}, 
% \end{eqnarray}
% where $i_{s}^{l,h}$ is the restoring restoration for masked privacy span $s$ on head $h$ in layer $l$, $\mathcal{S}$ is the total masked privacy span set and $\mathcal{I}_{l}^{h}$ is the meta restoration for head $h$ in layer $l$.

% An overview of PrivacyRestore is depicted in Figure \ref{fig:algorithm}.
% PrivacyRestore comprises three sub-modules, namely edited attention heads identification, Restoration  Vector Training and restoration aggregation.


\begin{figure*}[htbp]
\centering
\includegraphics[width=1\textwidth]{fig/algorithm.pdf}
\caption{
The PrivacyRestore framework consists of three procedures. 
(1) \textbf{Edited Attention Heads Identification.}
This procedure aims to identify the attention heads that, after being edited with restoration vectors, can achieve the most effective restoration effect.
Different privacy spans may require different attention heads for effective restoration. 
We propose top-K Heads Selector to obtain the common top-K heads set.  
(2) \textbf{Restoration Vectors Training.}
The training objective is to align the predictions given the input with privacy spans removed to be the same as the predictions given an intact input. 
Restoration vectors are trainable while LLM are frozen. 
(3) \textbf{Attention-aware Weighted Aggregation (AWA).} 
AWA is responsible for aggregating the restoration vectors of all privacy spans in the input and generating a meta restoration vector. 
This meta restoration vector is then utilized to edit the attention heads of the LLM. 
%It is calculated as a weighted sum of restoration vectors for all privacy spans. To assign weights, a smaller auxiliary model is employed to estimate the importance of each privacy span. 
During inference, the user sends a query with privacy spans removed, along with the meta restoration vector, to the server. 
}
\label{fig:algorithm}
\end{figure*}
%We employ the \textbf{Attention-aware Weighted Aggregation} method to generate the meta restoration vector for users. 
%We use the probe technique to obtain top-K heads set for each privacy span. 
% \revisezq{The highlight should be in yellow, red highlight hinders reading}
% %第一个panel，两个眼睛的logo不够醒目，闭上眼睛的logo的解释不是mask，是delete
% %第三个panel,应该显示把删除privaty spans的question写出来。



\subsection{Edited Attention Heads Identification} 
This procedure aims to identify the attention heads that, after being edited with restoration vectors, can achieve the most effective restoration effect.


% \begin{figure*}[htbp]

% \centering
% \includegraphics[width=0.2\textwidth]{fig/steering.pdf}
% \caption{
% }
% \label{fig:algorithm}
% \end{figure*}

% --------------------------------------------------------
% \revisezq{introduce edited attention heads.}
%介绍一下，这些attention heads要找出来，attention要加在上面。
% \begin{wrapfigure}{r}{0.4\textwidth} % r 表示图片在右侧, 0.4\textwidth 表示图片占据文本宽度的40%
%     \centering
%     \includegraphics[width=0.4\textwidth]{fig/steering.pdf} % 替换为你的图片文件名
%     \caption{示例图片}
% \end{wrapfigure}

According to \cite{elhage2021mathematical, vaswani2017attention}, the transformer architecture utilizes attention mechanism to capture the relationship between the current token and its surrounding context.
The attention mechanism can be expressed as:
\begin{eqnarray}
    \label{eq:MHA}
    \mathbf{U}^{l,h} &=& \text{Attn}^{l,h}(\mathbf{X}^{l,h}),
\end{eqnarray}
where $\mathbf{X}^{l,h}$ the sequence input of $h$-th head in the $l$-th layer and $\mathbf{U}^{l,h}$ is the sequence output. 
% $\mathbf{X}^{l,h}, \mathbf{U}^{l,h} \in \mathbb{R}^{\text{s} \times \text{h}}$, where $s$ is the sequence length and h is the dimision of  
Directly removing privacy spans may lead to insufficient relationships due to incomplete context and produce wrong head outputs.
Following activation steering methods \citep{li2023iti, chen2024truth}, we inject restoration vectors into the outputs of each attention head to restore private information:
\begin{eqnarray}
     % \label{eq:MHA-inter-2}
     % \mathcal{I}_{l}^{h} &=& \sum_{s\in\mathcal{S}}i_{s}^{l,h}, \\
     \label{eq:MHA-inter-1}
     % (\mathbf{u}^{l,h}, \mathbf{x}^{l,h}) &=& (\mathbf{U}^{l,h}[-1], \mathbf{X}^{l,h}[-1]) \\
     \mathbf{y}^{l,h} &=& \mathbf{u}^{l,h} + \mathcal{R}^{l, h},
     % \mathbf{u}^{l,h} &=& \text{Attn}^{l,h}(\mathbf{x}^{l,h}) + \mathcal{R}^{l, h}, 
\end{eqnarray}
where $\mathbf{u}^{l,h} = \mathbf{U}^{l,h}[-1]$ is the output of the last token and $\mathbf{y}^{l,h}$ is the output after privacy restoration.
%$\mathcal{S}$ is the total masked privacy span set and
$\mathcal{R}^{l, h}$ is the aggregated restoration vector for $h$-th head in $l$-th layer. 
The aggregated restoration vector is the aggregation of restoration vectors for all privacy spans in the user input, which will be introduced detailedly in \S \ref{sec:res_agg}
%$i_{s}^{l,h}$ is the restoring restoration vector for masked privacy span $s$ on head $h$ in layer $l$, 
%\revisezq{what is $i_{s}^{l,h}$?}


% --------------------------------------------------------



As pointed by activation steering methods \citep{li2023iti, chen2024truth}, applying restoration vectors to all attention heads in LLM will degrade the model performance.
% and only a subset of heads appear to be related to particular patients' privacy spans.
As shown in the first part of Figure \ref{fig:algorithm}, we employ the probe technique \cite{alain2016understanding, tenney2019bert, belinkov2022probing} to ascertain the most salient heads associated with each privacy span. 
We train a separate classifier for each head, tailored to each privacy span $s$, formulated as 
\begin{equation}
    \mathcal{F}_{s}^{l, h} (\textbf{u}^{l,h}) = \sigma (\theta \cdot \textbf{u}^{l,h}), 
\end{equation}
where $\textbf{y}^{l,h}$ is the output of the last token on $h$-th head of $l$-th layer,
and $\theta$ is the parameters of the classifier.
In our setting, the classifier is to discriminate whether the target privacy span $s$ appears in the query.
A classifier associated with an attention head demonstrating higher accuracy suggests a stronger correlation with the target privacy span, therefore, we select the top $K$ attention heads with high accuracies for each privacy span.


  % \begin{subfigure}[t]{0.46\textwidth}
  %   \includegraphics[width=1\textwidth]{fig/steering.pdf}
  %   \label{fig:steer}
  %   \subcaption{\revisezd{A sketch of injecting restoration vectors into a multi-head attention module.}}
  % \end{subfigure}
\begin{figure}[h]
  \begin{minipage}[t]{0.47\textwidth}
Considering the privacy protection scenario, using different top-K head sets for different privacy spans may suffer the risk of privacy leakage. 
If different privacy spans have different edited attention heads, the attacker can infer a specific privacy span based on some characteristics of attention heads. 
For example, an attacker might observe that only the heads set of privacy span ``\texttt{HIV}'' contains the $j$-th head and the appearance of $j$-th head indicates the presence of '\texttt{HIV}' in the user.
%例子描述得不太好，要用chatgpt润色。
We propose an algorithm named \textbf{Top-K Heads Selector} to combine all different top-K heads sets of all privacy spans to form a common top-K heads set $\mathcal{H}_c$ according to statistical characteristics.
Firstly, we initialize an empty score list $L_h$ for each head. 
Secondly, each privacy span $s$ has its corresponding top-K heads set $\mathcal{H}_k^s$. 
For each head $h$ in $\mathcal{H}_k^s$, we append score $K-\text{SortedIndex}(h, \mathcal{H}_k^s)$ into its score list $L_h$.
Thirdly, we calculate the average value of each score list $L_h$ as the score of the corresponding head.
Finally, we sort all heads in the LLM by the scores and pick up top-K heads as the common top-K heads set $\mathcal{H}_c$. 
The detailed algorithm is described in Algorithm \ref{alg:agg_head}.
  \end{minipage}
  \hfill % 添加水平填充
  \begin{minipage}[t]{0.50\textwidth}
        \raggedleft % 右对齐
        \begin{algorithm}[H] 
            \caption{Top-K Heads Selector}
            \label{alg:agg_head}
            \begin{flushleft}
                % \revisezq{
                \textbf{Input:} $\mathcal{S}$ is the set of privacy spans; $\mathcal{H}_a$ is the set of all heads; $\mathcal{H}_k$ is the set of top-K heads sets; 
                $\mathcal{H}_k^s$ is the top-K heads set of the symptom $s$; $\text{SortedIndex}(h, \mathcal{H}_{k}^s)$ is the function that sorts $\mathcal{H}_k^s$ in descending order based on the accuracy of the classifier for head $h$ and returns the index of $h$.
            \end{flushleft}
            \begin{algorithmic}[1]
                \STATE Initialize an empty score list $L_h = [\;]$ for each head $h$ in $\mathcal{H}_a$. \\
                 % // $\mathcal{H}_k^s$ is ordered descending order.
                \FOR{ $\mathcal{H}_k^s\;$ \text{in} $\;\mathcal{H}_k$} 
                    \FOR{$h\;$ \text{in} $\;\mathcal{H}_k^s$}
                    \STATE Append $K-\text{SortedIndex}(h, \mathcal{H}_k^s)$ into $L_h$.
                    \ENDFOR
                \ENDFOR
                 \FOR{$h\;$ \text{in} $\;\mathcal{H}_a$}
                   \item $\text{score}_h = \text{average}(L_h)$
                \ENDFOR
                \STATE Sort $\mathcal{H}_a$ according to $\text{score}_h$ and select top-K heads to obtain \textbf{common top-K heads set} $\mathcal{H}_c$.
            \end{algorithmic}
            \begin{flushleft}
                \textbf{Output:} $\mathcal{H}_c$ is the common top-K heads set.
            \end{flushleft}
        \end{algorithm}
  \end{minipage}
\end{figure}


\subsection{Restoration Vectors Training}
\label{sec:res_corr}

% --------------------------------------------------------------

%% bank constuction 计算restoration; 计算top head
%As shown in Equation \ref{eq:MHA-inter-1}, we need to compute restoration vector $i_{s}^{l,h}$ for each potential privacy span across various heads and layers. 
%As depicted in the left part of Figure\ref{fig:algorithm}, for each medical query $Q_{i}$ containing the target privacy span $s$: \textit{short of breath}, we generate one pair <$\widetilde{Q}_{i}, Q_{i}$> where $\widetilde{Q}_{i}$ represents the version with the privacy span masked, and $Q_{i}$ denotes the original query with no alterations.
%Both queries in the pair are fed into LLM and the inner hidden state of the last token \revisezd{for each} different heads and \revisezd{each} layers, $\widetilde{z_{l,i}^{h}} = \widetilde{x_{l,i}^{h}}[-1]$ and $z_{l,i}^{h} = x_{l,i}^{h}[-1]$, are recorded.
%Restoration vector of target privacy spans for head $h$ in layer $l$ can be computed as followed:
%\begin{equation}
%    \label{eq:restoration}
%    i_{s}^{l,h} = \sum_{i}(z_{l,i}^{h} - \widetilde{z_{l,i}^{h}}) / N,
%\end{equation}
%where $i_{s}^{l,h}$ is the restoring restoration vector for masked privacy span $s$ on head $h$ in layer $l$, $\mathcal{S}$ is the total masked privacy span set and N is the number of generated pairs for the target privacy spans. 
%We group each potential privacy span with its restoration vector to form Restore Bank.

% --------------------------------------------------------------

%% 训练restoration
Restoration vectors are designed to restore the information contained within the removed privacy spans. The training objective is to align the predictions given the input with privacy spans removed to be the same as the predictions given an intact input. 
%We propose a method for training restoration vectors using supervised fine-tuning (SFT). 
%However, directly injecting \revisezd{initial} restoration vectors \revisezd{potentially containing noise -> that are roughly computed} cannot achieve perfect alignment.

% \revisezq{diagnosis -> response, question -> query}
As illustrated in the second part of Figure \ref{fig:algorithm}, we generate training samples by appending gold response as the positive answer $a_p$ to user queries.
%\revisezd{We observed that the generation of the model includes some empty instances.}
The invasive injection of restoration vectors modifies the attention activation and may adversely affect the instruction-following capability of the LLM.
To maintain the instruction-following capability, we include an empty response as the negative answer $a_n$ for each sample.
Consequently, we obtain the training dataset $D = \{(q, a_p, a_n) | q \in Q, a_p \in A, a_n = \text{<EOS>} \} $, where $q$ denotes the query with privacy spans removed, $Q$ denotes the query set, $a_p$ denotes the positive answer, $A$ signifies the gold answer set,
$a_n$ denotes the negative answer, and <EOS> is the token indicating the end of a sequence.

For each privacy span $s \in \mathcal{S}$, there is a trainable restoration vector $r_{s}^{l,h}$  for each head $h$ in the common top-K heads set $\mathcal{H}_c$. 
Restoration vectors of all privacy spans are the only trainable parameters of our method. The LLM weights are frozen. Our method is plug-and-play and parameter-efficient for training. 
%\revisezd{\textbf{delete} Different from preview SFT methods, we fine-tune these restoration vectors rather than LLM itself to achieve restoration vector training.}
%\revisezd{To get better restoration vectors, we} fix all parameters in LLM excluding restoration vectors $I_{s}^{h}$ and initialize $I_{s}^{h}$ using $i_{s}^{l,h}$ computed by Equation \ref{eq:restoration} \revisezd{which is plug-and-play and parameter-efficient for training.}
%\revisezd{\textbf{delete} Focusing solely on the restoration vector significantly reduces the size of trainable parameters and decreases training costs.}
We fine-tune these restoration vectors using ORPO loss proposed by \cite{orpo}:
\begin{eqnarray}
    \label{eq:loss}
    \log P(a|q; \Theta) &=& \frac{1}{|a|}\sum_{i=1}^{|a|} \log (P(a|q; a_{<i}; \Theta)), \\
    \text{ratio}(a|q; \Theta) &=& \frac{P(a|q; r_s^{l,h})}{1-P(a|q; \Theta)},
    \\
    \mathcal{L}_{\text{ORPO}} &=& - \log P(a_p|q; \Theta) - \log \sigma \left( \log \frac{\text{ratio}(a_p|q; \Theta)}{\text{ratio}(a_n|q; \Theta)} \right),
\end{eqnarray}
where $q$ denotes the query with privacy spans removed, $\Theta$ is the set of restoration vectors corresponding to the privacy spans present in the input..
$a$ is a response, which can be positive response $a_p$ or negative response $a_n$. $|a|$ is the length of the response. 
% \revisezq{$r^{l,h}_{s}$ is the vecotr of a single span. $q$ has multiple spans.}
% Subscript $p,n$ indicates the positive or negative one. 
$\mathcal{L}_{\text{ORPO}}$ simultaneously encourages generating correct responses and diminishes the occurrence of meaningless empty responses. 
%During training, given a query $q$ with all privacy spans removed and the set of removed spans is denoted as $\mathcal{S}_q$, the restoration vector $r^{l,h}_s$ of each privacy span $s \in \mathcal{S}_q$ will be optimized.
%\revisejw{After training, we obtain the optimized restoration vectors for each privacy span, as shown in the second part of Figure \ref{fig:algorithm}. }
% After training, we obtain the restoration bank which consists of restoration vectors for each privacy span and the common top-K head set.
% 训练时把所有span都删除
%Finally, we obtain these corrected restoration vectors, denoted as $IC_{s}^{h}$.


\subsection{Attention-aware Weighted Aggregation}
\label{sec:res_agg}
%% weighted aggregation
%The aforementioned processes aim at obtaining the restoration vectors $IC_{s}^{h}$, which are subsequently utilized to restore masked privacy spans for the purpose of privacy protection. 
%As shown in the right part of Figure \ref{fig:algorithm}, \revisezd{user inputs often contain multiple privacy spans. 
%Certain privacy spans may exert a critical influence on response, while others may not be as significant.
There are commonly multiple privacy spans that may lead to privacy leakage in user inputs.
% We should aggregate corresponding restore vectors and send the aggregated results to the server to prevent attacks and identify the restore vectors and privacy span. 
Some of privacy spans may have a critical impact on final outputs, while others may not be as significant.
Directly aggregating all restoration vectors equally may weaken the impact of the critical privacy spans and enlarge the impact of irrelevant privacy spans.
% \revisezq{see Chinese comments.}
% 无关紧要的privacy span会干扰。
Therefore, we propose a novel method called \textbf{Attention-aware Weighted Aggregation (AWA)} which estimates a weight for each privacy span, and then takes the weighted sum of restoration vectors as the aggregation. 
%{which distinguishes important privacy spans with the help of tiny models}.
% 为什么要命名为Collaborative. 
% 是小模型和大模型协作。
To discern the importance of different privacy spans and consider the limitations of computing resources, we employed a tiny model (such as BERT \cite{devlin2019bert}) on the client side to calculate the importance weights.
% \revisezd{\textbf{delete} given constraints on computing resources.}

As depicted in the third panel in Figure \ref{fig:algorithm}, the first step of AWA is 
%utilizing an attention mechanism 
computing attention score of the last token $t$ attending to a privacy span $s$, yielding importance weights denoted as $w_s$:
% \revisezq{revise equation}
% W_Q, W_K的字母加下标，token t对应的x
\begin{eqnarray}
    \label{eq:loss}
    \text{Attn}^{h}(s_{j}, x_t) &=& \text{Softmax}(x_t \mathbf{W}_{Q}^{h} \cdot (s_{j} \mathbf{W}_{K}^{h})^{T}), \\
    w_s &=& \frac{1}{|s|} \sum_{j=1}^{|s|}\frac{1}{|H|}\sum_{h \in H}\text{Attn}^{h}(s_{j}, x_t),
\end{eqnarray}
where 
%the upper script $h$ denotes the head $h$, 
$\mathbf{W}_{Q}^{h}$ and $\mathbf{W}_{V}^{h}$ are the query and key projection matrices of head $h$ in the last layer of a tiny model, respectively. 
% \revisezq{last layer}
$x_t$ and $s_{j}$ represents the hidden state of the last token $t$ and the $j$-th token of privacy span $s$ in the last layer, respectively. 
%$H$ is a set of attention heads in the last layer of the tiny model and 
$H$ denotes all attention heads in the last layer. 
$|s|$ denotes the number of tokens contained in $s$.

After obtaining importance weights of multiple privacy spans in the query, we calculate the aggregated restoration vector $\mathcal{R}^{l, h}$ of the $l$-th layer and $h$-th head as follows, 
\begin{eqnarray}
     \label{eq:newComplex}
     \mathcal{R}^{l, h} &=&
     \begin{cases} 
     r_{s}^{l,h} + \epsilon & \text{if } |\mathcal{S}_q| = 1, \\
      \sum_{s\in\mathcal{S}_q} w_s \cdot r_{s}^{l,h} & \text{otherwise },
   \end{cases}
\end{eqnarray}

where $\mathcal{S}_q$ denotes the privacy spans containing in the query and $|\mathcal{S}_q|$ is the number of privacy spans. 
In the scenario where the query contains a single privacy span, the aggregated restoration vector is the restoration vector $r_{s}^{l,h}$ itself.
An attacker can intercept $\mathcal{R}^{l, h}$ and easily deduce the plain text of the privacy span.
We inject noise $\epsilon$ into the restoration vector, making it difficult for attackers to infer the plain text of privacy span from $\mathcal{R}^{l, h}$.
% \revisezq{why?}


The client side maintains a local \textbf{Restoration Bank} responsible for providing the meta restoration vector based on a given query and a set of privacy spans. 
The Restoration Bank comprises three key components: the aggregation algorithm AWA, restoration vectors for each privacy span, and a common top-K heads set. 
The meta restoration vector can be obtained by concatenating the $\mathcal{R}^{l,h}$ for all heads in the common top-K heads set. 
The server is aware of the specific order of concatenation.
%which is responsible for retrieving restoration vectors corresponding to privacy spans, aggregating them into aggregated restoration vectors by using a tiny model, and gathering aggregated vectors as a meta restoration vectors. 
 

% \revisejw{We obtain the meta restoration vector $\mathcal{R}$ by gathering aggregated vectors $\mathcal{R}^{l, h}$ for all heads in $\mathcal{H}_c$.}
% \revisezq{Then the client side sends the meta restoration vectors $\mathcal{R}^{l,h}$ and the query with privacy spans removed to the server side.
% The server side conducts privacy restoration during LLM inference, as shown in the third part of Figure \ref{fig:algorithm}.}
% \revisezq{what is the meta?,what is restoration bank?}
% bank 包括聚合的算法
%直接说meta是什么。

% CIO evaluates the importance measure of privacy spans when aggregating multiple restoration vectors in comparison to the initial version defined in Equation \ref{eq:MHA-inter-2}.

% \revisezq{single vector adds noise.}

% \revisezq{add another section: Inference}
% 用户可以自定义span


\subsection{Inference}
\label{sec:infer}
% 用户可以自定义span
% 只返回meta vector
% 每个head位置都返回一个i vector


% 用户输入查询，自定义 span
As depicted in the third panel of Figure \ref{fig:algorithm}, during LLM inference, on the client side, users are allowed to select specific spans (e.g., \texttt{black stools, pale skin, blood in stool}) which they wish to keep undisclosed.
These selected spans are considered as privacy spans. 
% 客户端从 bank 检索 vector，并使用小模型聚合 meta
% from the restoration bank
% 直接说从 bank 得到什么
% \revisezq{The the client side retrieves restoration vectors corresponding to these privacy spans and aggregates them into the meta restoration vector using a tiny model.}
The client side obtains the meta restoration vector from the Restoration Bank.
% 客户端提供删除 span 的查询和 meta vector
Then, the client side provides queries with privacy spans removed and the meta restoration vector to LLMs deployed on the server side. 
% 服务器端注入 meta vector
On the server side, the meta restoration vector will be injected into attention heads of LLMs in the common top-K heads set. 
% 客户端接收输出
Finally, the client receives response outputs generated by the LLM.




% \subsection{Defense to Various Attacks}
% \label{sec:defense}
% % 被攻击的点
% % 再说不会被攻击
% % (1) attack: meta restoration is incepted. 
% % defense: 单个向量加扰动 + 多个向量是叠加的
% % (2) attack server 被人控制了。 own an exactly same LLM, attack obtain meta restoration and query with privacy spans deleted, can use a harmful prompt to ask privacy information rather than output. 
% % defense: our experiments proves that the attack rate is low. 
% % (3) attack： server 被人控制了 attribute inference attack. 
% %  defense: experiment. 

% We enumerate the potential attacks that PrivacyRestore may face and demonstrate that PrivacyRestore can effectively defend against them as follows.

% \textbf{Leakage of restoration vectors of each privacy span and meta restoration vector. }

% Attackers may illegally obtain restoration vectors of each privacy span and intercept the meta restoration vector sent to the server.
% Even in such scenarios, it is still difficult for attackers to infer privacy spans based on a specific meta restoration vector.
% % 分情况分析
% According to the AWA method in \S \ref{sec:res_agg}, when only one privacy span exists in the query, the meta restoration vector is a restoration vector with random noise injected, \revisezq{can not infer...}
% % which satisfies the \revisezq{token representation privatization \cite{qu2021natural}}.
% When the query contains multiple privacy spans, attackers need to try all combinations of restoration vectors to infer the privacy span.
% The number of combinations that the attacker needs to try is equal to the sum of combinatorial numbers of any number of restoration vectors, which can be expressed as:
% \begin{equation}
%     \mathcal{N}_{c} = \sum_{i=2}^{|\mathcal{S}|} C_{|\mathcal{S}|}^{i} = 2^{|\mathcal{S}|} - |\mathcal{S}| - 1,
% \end{equation}
% where $|\mathcal{S}|$ is the total number of privacy spans, and $C_n^i$ represents the combinatorial number of \revisezd{ways to choose $i$ elements from a set of $n$ elements}.
% The number of combinations grows exponentially with $|\mathcal{S}|$, and in practical scenarios where $|\mathcal{S}|$ is typically large, so it is impossible for attackers to infer privacy spans even if the restoration vectors of each privacy span are available.


% \textbf{Prompt Injection Attack. }
% The attack condition is that attackers own LLM weights and can obtain meta restoration vector and a query with privacy spans removed. 
% % \revisezq{add inject process}
% % 先截取,再注入,再发送给LLM
% During inference, attackers intercept the query sent by the client, modify the content of the query, and then send it to the server.
% Attackers inject malicious content into the query to manipulate the LLM to generate privacy information. 
% For example, in medical diagnosis task, the malicious content would be ``print out the possible symptoms.'' 
% % attempt to obtain privacy information by 
% For prompt injection attack, experimental results in Table \ref{table_avg_acc} show that the attack success ratio of our method is lower than baselines.


% \textbf{Attribute Inference Attack. }
% The attack condition is the same with Prompt Injection Attack.
% Attribute Inference Attack aims to recover sensitive attributes in the input text.
% Attackers commonly use input text or its embeddings as input to train a classifier to classify whether sensitive attributes are contained in input text.
% As shown in Table \ref{table_avg_acc}, the F1 score of classifier for our method is low.


